Entity-Centric Query Refinement

We introduce the task of entity-centric query refinement. Given an input query whose answer is a (potentially large) collection of entities, the task output is a small set of query refinements meant to assist the user in efficient domain exploration and entity discovery. We propose a method to create a training dataset for this task. For a given input query, we use an existing knowledge base taxonomy as a source of candidate query refinements, and choose a final set of refinements from among these candidates using a search procedure designed to partition the set of entities answering the input query. We demonstrate that our approach identifies refinement sets which human annotators judge to be interesting, comprehensive, and non-redundant. In addition, we find that a text generation model trained on our newly-constructed dataset is able to offer refinements for novel queries not covered by an existing taxonomy. Our code and data are available at https://github.com/google-research/language/tree/master/language/qresp.

==> algo/search.tex <==
\begin{algorithm}[t]
    \caption{Entity-centric exploratory search}
    \label{algo:search}
    \begin{algorithmic}
        \Procedure{DiscoveryEntity}{$q, k, T$}
        \While{$|\cA(q)| > T$}
        \State Model makes $k$ refinements $\cR(q)$.
        \State User selects a $q'_i \in \cR(q)$.
        \State $q \gets q'_i$
        \EndWhile
        \State User selects a final entity $q*$ from $\cA(q)$.
        \State \textbf{return} $q*$
        \EndProcedure
    \end{algorithmic}
\end{algorithm}


==> appx_correction.tex <==
\section{Refinement correction} \label{appx:correction}

Table \ref{tbl:correction_counts} shows confusion matrices comparing human relevance judgments with relevance predictions from $\Aml$ on YAGO and NQ-TREC. 

\input{table/correction_counts.tex}


==> appx_results.tex <==
\section{Additional results}

\subsection{Additional filtering steps}

We perform a few additional filtering steps to remove uninteresting suggestions: we run a Spacy NER tagger and remove refinements with named entities from the following categories: ["DATE", "GPE", "NORP", "LOC"]. We do a ``diff'' for this; if the entity appeared in the query, we keep it. Only remove if it's in the refinement only. Finally, we remove a handful of additional terms: ``men'', ``women'', ``male'', ``female'', and regular expressions matching centuries like ``$13^{th}$ century''.

\djw{Give some more stats about yago. How many total categories, how many we kept, etc.See the YAGO stats section of the commands file.}

\input{table/yago_counts_wrapper.tex}.

\subsection{Taxonomy-provided refinements}


Table \ref{tbl:ab_gold_filter_best_filter_random} shows A / B tests comparing best with random selection, when using filtered data for both. The numbers aren't quite as strong as in Table \ref{tbl:ab_gold_filter_best_all_random}, but still heavily favor our selection method.

\input{table/ab-gold-filter_best-filter_random-wrapper.tex}

\subsection{Taxonomy-free refinements}

Table \ref{tbl:ab_yago_best_filter_random} shows that it's not just the filtering; our data selection method still helps post-filtering. 

\input{table/ab-yago-best-filter_random_wrapper.tex}


TODO make show to include the results with answer entities vs. not.


==> sec_correction.tex <==
\section{Refinement correction} \label{sec:correction}

The results of the previous section suggest that $\Msys$ refinements decrease in relevance under domain shift.  As a step toward addressing this challenge, we return to the idea that motivated \sysname: use the entities answering the candidate refinements to guide the refinement selection process. In \S \ref{sec:method}, we made use of gold entities $\cA(q)$ found in a knowledge base. Here, we use an off-the-shelf machine learning model $\Aml(q)$ to predict answers for novel queries.

\paragraph{Question answering model: RELIC}

We use the RELIC model \cite{Ling2020LearningCE} as our QA system $\Aml$. RELIC uses a dual-encoder architecture consisting of (1) learned embeddings $f(e_i)$ for all entities in Wikipedia, and (2) an encoder $g(q)$ mapping an input query $q$ to a shared embedding space. RELIC encodes $q$ using $g(q)$, then ranks all entities $f(e_i)$ based on their cosine similarity to $g(q)$, and returns all entities with similarity higher than a threshold $t$ as answers to $q$. We finetune RELIC on the YAGO train set from \S \ref{sec:dataset_creation}, training for 310,000 steps with a batch size of 1024 and learning rate of $1 \times 10^{-4}$. A single training instance consists of a query $q$, paired with an answer $e_i \in \cA(q)$; all other entities in the batch are used as negatives. We set $t=0.4$ based on performance on a held-out portion of the train set. This gives precision, recall, and F1 of 23.7, 51.9, and 32.6 respectively. 

\paragraph{Identifying irrelevant refinements}

To identify refinements $q'_i$ likely to be irrelevant to the original query $q$, we adopt the following heuristic: predict $q'_i$ as irrelevant if $q'_i$ and $q$ share no answers -- i.e. $\Aml(q'_i) \cap \Aml(q) = \emptyset$. In principle, each $q'_i$ should meet the stricter requirement $\Aml(q'_i) \subseteq \Aml(q)$, but this may not be satisfied for valid refinements since the predictions from $\Aml$ are not perfectly accurate.

% A refinement $q'_i$ is considered relevant if it is a subtype of $q$ -- i.e. $\cA(q'_i) \subseteq \cA(q)$. In cases where we do not have access to ``gold'' answers, we can use predicted answers from $\Aml$ to identify refinements likely to be judged as irrelevant. Since these predictions may be noisy, only keeping refinements whose predicted answers $\Aml(q'_i)$ are a strict subset of $\Aml(q)$ is likely to be overly stringent. We err on the side of leniency, and predict a refinement to be irrelevant if its answers have \emph{no} overlap with the answers to the original query.

Applying our heuristic, 42\% of YAGO refinements marked irrelevant by humans were (correctly) flagged by $\Aml$ as irrelevant, whereas only 10\% of refinements marked relevant by humans were (incorrectly) flagged by $\Aml$. For \nqtrec, these percentages are 22\% and 7.8\%, respectively. In both cases, there is a statistically significant association between the model's predictions and human judgments ($p < 10^{-10}$, $\chi^2$ test). However, the association is relatively weak: using our heuristic as a classifier to predict irrelevant refinements achieves F1 scores of 29.6 and 30.0 on YAGO and NQ-TREC, respectively. \djw{See Appendix \ref{appx:correction} for full confusion matrices.}

We also experimented with using predicted answers from $\Aml$ to score entire RSs according to Eq. \ref{eqn:cost}. The resulting scores had little association with human judgments, likely due to the accuracy limitations of $\Aml$ on this task. 


==> table/ab-gold-filter_best-all_random-wrapper.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \input{table/human_evals/ab-gold-filter_best-all_random.tex}
    \caption{Human evaluations}
    \label{tbl:ab_gold_filter_best_all_random}
\end{table}


==> table/ab-gold-filter_best-filter_random-wrapper.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \input{table/human_evals/ab-gold-filter_best-filter_random.tex}
    \caption{Human evaluations in taxonomy-provided setting}
    \label{tbl:ab_gold_filter_best_filter_random}
\end{table}


==> table/ab-yago-best-all_random_wrapper.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \input{table/human_evals/ab-yago-filter_joint_best_gold_false-all_joint_random_gold_false.tex}
    \caption{Human evaluations comparing best with random}
    \label{tbl:ab_yago_best_all_random}
\end{table}


==> table/ab-yago-best-filter_random_wrapper.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \input{table/human_evals/ab-yago-filter_joint_best_gold_false-filter_joint_random_gold_false.tex}
    \caption{Human evaluations in taxonomy-free setting}
    \label{tbl:ab_yago_best_filter_random}
\end{table}


==> table/ab-yago-sequential-independent_wrapper.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \input{table/human_evals/ab-yago-filter_joint_best_gold_false-filter_separate_best_gold_false.tex}
    \caption{Human evaluations comparing sequential vs. independent prediction}
    \label{tbl:ab_yago_sequential_independent}
\end{table}


==> table/auto_evals/automated_metrics_orig.tex <==
\begin{tabular}{lllllrrrrrrrr}
\toprule
  data & filter &  generation &   answers & decoding &  bleu &  rouge1 &  rouge2 &  rougeL &  precision &  recall &   f1 &  perplexity \\
\midrule
  Best & \cmark &  Sequential &      None &   Greedy &  67.1 &    73.3 &    57.6 &       69.4 &       24.8 &    24.3 & 24.6 &        2.01 \\
  Best & \cmark &  Sequential &      None &   Sample &  67.2 &    72.9 &    57.3 &       68.7 &       23.5 &    23.3 & 23.4 &        2.01 \\
  Best & \cmark &  Sequential &      Gold &   Greedy &  73.9 &    78.5 &    65.1 &       74.9 &       35.2 &    34.4 & 34.8 &        1.86 \\
  Best & \cmark &  Sequential & Predicted &   Greedy &  68.2 &    74.8 &    58.3 &       68.7 &       22.8 &    22.2 & 22.5 &        2.73 \\
  Best & \cmark & Independent &      None &   Sample &  66.9 &    72.7 &    56.4 &       68.2 &       19.6 &    19.2 & 19.4 &        2.35 \\
  Best & \xmark &  Sequential &      None &   Greedy &  60.0 &    68.6 &    49.3 &       65.3 &       13.1 &    13.0 & 13.1 &        2.10 \\
Random & \cmark &  Sequential &      None &   Greedy &  61.5 &    69.4 &    51.2 &       66.0 &       15.1 &    14.3 & 14.7 &        2.11 \\
Random & \xmark &  Sequential &      None &   Greedy &  57.6 &    66.5 &    46.2 &       63.8 &        6.8 &     6.7 &  6.8 &        2.19 \\
\bottomrule
\end{tabular}


==> table/correction_counts.tex <==
\begin{table}[t]
    \footnotesize
    \centering

    \begin{subtable}[h]{\linewidth}

        \begin{tabular}{ll|cc|cc}
            \multicolumn{2}{c}{}            & \multicolumn{3}{c}{\textbf{Predicted}} &                         \\
            \multicolumn{2}{c|}{}           & Irrelevant                             & Relevant & Total        \\
            \cmidrule(lr){2-5}
            \multirow{3}{*}{\textbf{Human}} & Irrelevant                             & 91       & 128   & 219  \\
                                            & Relevant                               & 304      & 2642  & 2946 \\
            \cmidrule(lr){2-5}
                                            & Total                                  & 395      & 2770  & 3165 \\
        \end{tabular}

        \caption{YAGO}
        \label{tbl:correction_yago}
    \end{subtable}

    \begin{subtable}[h]{\linewidth}

        \begin{tabular}{ll|cc|cc}
            \multicolumn{2}{c}{}            & \multicolumn{3}{c}{\textbf{Predicted}} &                         \\
            \multicolumn{2}{c|}{}           & Irrelevant                             & Relevant & Total        \\
            \cmidrule(lr){2-5}
            \multirow{3}{*}{\textbf{Human}} & Irrelevant                             & 97       & 349   & 446  \\
                                            & Relevant                               & 104      & 1236  & 1340 \\
            \cmidrule(lr){2-5}
                                            & Total                                  & 201      & 1585  & 1786 \\
        \end{tabular}

        \caption{\nqtrec}
        \label{tbl:correction_nq}
    \end{subtable}

    \caption{Confusion matrices comparing human vs. predicted judgments of refinement relevance. The rows provide counts for refinements judged (ir)relevant by human annotators. The columns show model predictions.}

    \label{tbl:correction_counts}

\end{table}


==> table/human_evals/_new_ab-gold-filter_best-all_random.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Best vs. \textbf{B} = Random} \\
\midrule
          N = 105 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &               98\% &     0\% &               97\% \\
\cmidrule(lr){1-4}
    Comprehensive &      \textbf{88\%} &    10\% &                2\% \\
      Informative &      \textbf{71\%} &    26\% &                3\% \\
    Non-redundant &                  - &       - &                  - \\
\cmidrule(lr){1-4}
          Overall &      \textbf{86\%} &    10\% &                4\% \\
\bottomrule
\end{tabular}



==> table/human_evals/_new_ab-gold-filter_best-filter_random.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Best vs. \textbf{B} = Random (filtered)} \\
\midrule
          N = 105 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &              100\% &     0\% &              100\% \\
\cmidrule(lr){1-4}
    Comprehensive &      \textbf{75\%} &    15\% &               10\% \\
      Informative &      \textbf{64\%} &    24\% &               12\% \\
    Non-redundant &                  - &       - &                  - \\
\cmidrule(lr){1-4}
          Overall &      \textbf{73\%} &    17\% &               10\% \\
\bottomrule
\end{tabular}



==> table/human_evals/_new_ab-nq-all_joint_best_gold_false-all_joint_random_gold_false.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Best (unfiltered) vs. \textbf{B} = Random} \\
\midrule
           N = 93 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &               75\% &     0\% &      \textbf{80\%} \\
\cmidrule(lr){1-4}
    Comprehensive &               30\% &    41\% &               29\% \\
      Informative &               20\% &    45\% &      \textbf{35\%} \\
    Non-redundant &               11\% &    67\% &      \textbf{23\%} \\
\cmidrule(lr){1-4}
          Overall &               26\% &    41\% &      \textbf{33\%} \\
\bottomrule
\end{tabular}


==> table/human_evals/_new_ab-nq-filter_joint_best_gold_false-all_joint_random_gold_false.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Best vs. \textbf{B} = Random} \\
\midrule
           N = 93 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &               56\% &     0\% &      \textbf{81\%} \\
\cmidrule(lr){1-4}
    Comprehensive &      \textbf{45\%} &    30\% &               26\% \\
      Informative &      \textbf{40\%} &    34\% &               26\% \\
    Non-redundant &               23\% &    51\% &      \textbf{26\%} \\
\cmidrule(lr){1-4}
          Overall &      \textbf{43\%} &    28\% &               30\% \\
\bottomrule
\end{tabular}


==> table/human_evals/_new_ab-yago-filter_joint_best_gold_false-all_joint_random_gold_false.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Best vs. \textbf{B} = Random} \\
\midrule
          N = 107 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &               93\% &     0\% &     \textbf{100\%} \\
\cmidrule(lr){1-4}
    Comprehensive &      \textbf{77\%} &    12\% &               11\% \\
      Informative &      \textbf{70\%} &    22\% &                8\% \\
    Non-redundant &      \textbf{22\%} &    66\% &               12\% \\
\cmidrule(lr){1-4}
          Overall &      \textbf{76\%} &    17\% &                7\% \\
\bottomrule
\end{tabular}



==> table/human_evals/_new_ab-yago-filter_joint_best_gold_false-filter_joint_best_gold_true.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Unconditional vs. \textbf{B} = Conditioned on answers} \\
\midrule
          N = 105 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &               94\% &     0\% &      \textbf{99\%} \\
\cmidrule(lr){1-4}
    Comprehensive &               45\% &    11\% &               44\% \\
      Informative &      \textbf{32\%} &    44\% &               24\% \\
    Non-redundant &      \textbf{21\%} &    65\% &               13\% \\
\cmidrule(lr){1-4}
          Overall &      \textbf{48\%} &    17\% &               35\% \\
\bottomrule
\end{tabular}



==> table/human_evals/_new_ab-yago-filter_joint_best_gold_false-filter_joint_random_gold_false.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
  \toprule
  \multicolumn{4}{c}{\textbf{A} = Best vs. \textbf{B} = Random (filtered)} \\
  \midrule
  N = 107           & \textbf{A} & Neutral & \textbf{B}    \\
  \midrule
  Fluent + Relevant & \textbf{94\%}      & 0\%     & 92\%                  \\
  \cmidrule(lr){1-4}
  Comprehensive     & \textbf{59\%}      & 21\%    & 20\%                  \\
  Informative       & \textbf{39\%}      & 35\%    & 26\%                  \\
  Non-redundant     & \textbf{23\%}      & 62\%    & 15\%                  \\
  \cmidrule(lr){1-4}
  Overall           & \textbf{59\%}      & 23\%    & 18\%                  \\
  \bottomrule
\end{tabular}


==> table/human_evals/_new_ab-yago-filter_joint_best_gold_false-filter_separate_best_gold_false.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Sequential vs. \textbf{B} = Independent} \\
\midrule
          N = 107 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &               93\% &     0\% &      \textbf{95\%} \\
\cmidrule(lr){1-4}
    Comprehensive &      \textbf{47\%} &    20\% &               33\% \\
      Informative &               28\% &    45\% &               27\% \\
    Non-redundant &      \textbf{42\%} &    45\% &               14\% \\
\cmidrule(lr){1-4}
          Overall &      \textbf{46\%} &    26\% &               28\% \\
\bottomrule
\end{tabular}



==> table/human_evals/ab-gold-filter_best-filter_random.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = \sysname vs. \textbf{B} = \filtername} \\
\midrule
          N = 105 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &                0\% &   100\% &                0\% \\
\cmidrule(lr){1-4}
    Comprehensive &      \textbf{75\%} &    15\% &               10\% \\
      Interesting &      \textbf{64\%} &    24\% &               12\% \\
    Non-redundant &                  - &       - &                  - \\
\cmidrule(lr){1-4}
          Overall &      \textbf{73\%} &    17\% &               10\% \\
\bottomrule
\end{tabular}


==> table/human_evals/ab-nq-all_joint_best_gold_false-all_joint_random_gold_false.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Best (unfiltered) vs. \textbf{B} = Random} \\
\midrule
           N = 93 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &                4\% &    87\% &       \textbf{9\%} \\
\cmidrule(lr){1-4}
    Comprehensive &               30\% &    41\% &               29\% \\
      Interesting &               20\% &    45\% &      \textbf{35\%} \\
    Non-redundant &               11\% &    67\% &      \textbf{23\%} \\
          Overall &               26\% &    41\% &      \textbf{33\%} \\
\bottomrule
\end{tabular}


==> table/human_evals/ab-yago-filter_joint_best_gold_false-all_joint_random_gold_false.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = \sysname vs. \textbf{B} = Random} \\
\midrule
          N = 107 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &                0\% &    93\% &       \textbf{7\%} \\
\cmidrule(lr){1-4}
    Comprehensive &      \textbf{77\%} &    12\% &               11\% \\
      Interesting &      \textbf{70\%} &    22\% &                8\% \\
    Non-redundant &      \textbf{22\%} &    66\% &               12\% \\
\cmidrule(lr){1-4}
          Overall &      \textbf{76\%} &    17\% &                7\% \\
\bottomrule
\end{tabular}


==> table/human_evals/ab-yago-filter_joint_best_gold_false-filter_joint_best_gold_true.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = Unconditional vs. \textbf{B} = Conditioned on answers} \\
\midrule
          N = 105 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &                1\% &    93\% &       \textbf{6\%} \\
\cmidrule(lr){1-4}
    Comprehensive &               45\% &    11\% &               44\% \\
      Interesting &      \textbf{32\%} &    44\% &               24\% \\
    Non-redundant &      \textbf{21\%} &    65\% &               13\% \\
\cmidrule(lr){1-4}
          Overall &      \textbf{48\%} &    17\% &               35\% \\
\bottomrule
\end{tabular}


==> table/human_evals/ab-yago-filter_joint_best_gold_false-filter_separate_best_gold_false.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
  \toprule
  \multicolumn{4}{c}{\textbf{A} = Sequential vs. \textbf{B} = Separate} \\
  \midrule
  N = 107           & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
  \midrule
  Fluent + Relevant & 3\%                & 92\%    & \textbf{6\%}       \\
  \cmidrule(lr){1-4}
  Comprehensive     & \textbf{47\%}      & 20\%    & 33\%               \\
  Interesting       & \textbf{28\%}      & 45\%    & 27\%               \\
  Non-redundant     & \textbf{42\%}      & 45\%    & 14\%               \\
  \cmidrule(lr){1-4}
  Overall           & \textbf{46\%}      & 26\%    & 28\%               \\
  \bottomrule
\end{tabular}


==> table/human_evals/gold-filter_best-all_random.tex <==
\begin{tabular}{L{7.2em} *{3}{R{3.9em}}}
\toprule
\multicolumn{4}{c}{\textbf{A} = \sysname vs. \textbf{B} = Random} \\
\midrule
          N = 105 & Prefers \textbf{A} & Neutral & Prefers \textbf{B} \\
\midrule
Fluent + Relevant &                3\% &    95\% &                2\% \\
\cmidrule(lr){1-4}
    Comprehensive &      \textbf{88\%} &    10\% &                2\% \\
      Interesting &      \textbf{71\%} &    26\% &                3\% \\
    Non-redundant &                  - &       - &                  - \\
\cmidrule(lr){1-4}
          Overall &      \textbf{86\%} &    10\% &                4\% \\
\bottomrule
\end{tabular}


==> table/human_evals/kappa.tex <==
\begin{tabular}{lr}
\toprule
{} &     0 \\
\midrule
fluent            &  0.37 \\
relevant          &  0.61 \\
comprehensiveness &  0.53 \\
informativeness   &  0.46 \\
non\_redundancy    &  0.39 \\
overall           &  0.52 \\
\bottomrule
\end{tabular}


==> table/yago_counts.tex <==
\begin{tabular}{lrr}
\toprule
{} &    all &  filter \\
fold  &        &         \\
\midrule
train &  17589 &    8958 \\
dev   &    298 &     282 \\
\bottomrule
\end{tabular}


==> table/yago_counts_wrapper.tex <==
\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.3em}
  \centering

  \input{table/yago_counts.tex}

  \vspace{1em}

  \caption{Yago dataset counts by fold}

  \label{tbl:yago_counts}

\end{table}

